From a Social Cognitive Perspective: Context-aware Visual Social Relationship Recognition

People's social relationships are often manifested through their surroundings, with certain objects or interactions acting as symbols for specific relationships, e.g., wedding rings, roses, hugs, or holding hands. This brings unique challenges to recognizing social relationships, requiring understanding and capturing the essence of these contexts from visual appearances. However, current methods of social relationship understanding rely on the basic classification paradigm of detected persons and objects, which fails to understand the comprehensive context and often overlooks decisive social factors, especially subtle visual cues. To highlight the social-aware context and intricate details, we propose a novel approach that recognizes \textbf{Con}textual \textbf{So}cial \textbf{R}elationships (\textbf{ConSoR}) from a social cognitive perspective. Specifically, to incorporate social-aware semantics, we build a lightweight adapter upon the frozen CLIP to learn social concepts via our novel multi-modal side adapter tuning mechanism. Further, we construct social-aware descriptive language prompts (e.g., scene, activity, objects, emotions) with social relationships for each image, and then compel ConSoR to concentrate more intensively on the decisive visual social factors via visual-linguistic contrasting. Impressively, ConSoR outperforms previous methods with a 12.2\% gain on the People-in-Social-Context (PISC) dataset and a 9.8\% increase on the People-in-Photo-Album (PIPA) benchmark. Furthermore, we observe that ConSoR excels at finding critical visual evidence to reveal social relationships.

==> chapters/06_bio.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{authors/wushiwei.pdf}}]{Shiwei Wu} received the B.E. degree in from the Xiamen University (XMU), Xiamen, China, in 2018. He is currently working towards the Ph.D. degree in University of Science and Technology of China (USTC), Hefei, China. He is working with Key Laboratory of Big Data Analysis and Application. His major research interests include social relationship recognition and large multimodal models.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{authors/zhangchao.pdf}}]{Chao Zhang} received the B.E. degree in software engineering from Shandong University, Jinan, China, in 2022. He is currently pursuing the M.S. degree with the  School of Computer Science and Technology, University of Science and Technology of China, Hefei, China.
He has authored or coauthored several papers in refereed conference proceedings, such as TKDE, CIKM and SIGIR.  His research interests include data mining, multimodal learning, and large language models.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{authors/joyachen.pdf}}]{Joya Chen} is a Ph.D. candidate at Show Lab, National University of Singapore. He received M.Sc. from University of Science and Technology of China. Currently, he is a research intern at FAIR, Meta AI. Previously he also worked with researchers from Reality Labs Research, Meta. His research focuses large multimodal models, particularly learning them for real-time, streaming video. 
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{authors/tongxu.jpeg}}]{Tong Xu}
 (Member, IEEE) is currently working as a Professor at University of Science and Technology of China (USTC), Hefei, China. He has authored more than 100 top-tier journal and conference papers in related fields, including TKDE, TMC, TMM, TOMM, KDD, SIGIR, WWW, ACM MM, etc. He was the recipient of the Best Paper Award of KSEM 2020, and the Area Chair Award for NLP Application Track of ACL 2023.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{authors/wulikang.pdf}}]{Likang Wu} is currently a Ph.D. candidate in the School of Computer Science and Technology at University of Science and Technology of China (USTC), P.R. China. His major research interests include recommendation system, graph embedding, and large language model. He has published several papers in refereed journals and conference proceedings. 
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./authors/chenenhong.pdf}}]{Enhong Chen} (Fellow, IEEE) is a professor and vice dean of the School of Computer Science at USTC. He received the Ph.D. degree from USTC. His general area of research includes data mining and machine learning, social network
analysis and recommender systems. He has published more than 100 papers in refereed conferences and journals, including IEEE Trans. KDE, IEEE Trans. MC, KDD, ICDM, NIPS, and CIKM. He was on program committees of numerous conferences including KDD, ICDM, SDM. His research is supported by the National Science Foundation for Distinguished Young Scholars of China. He is a fellow of the IEEE.
\end{IEEEbiography}
